MOROCCO: Model Resource Comparison Framework

The new generation of pre-trained NLP models push the SOTA to the new limits, but at the cost of computational resources, to the point that their use in real production environments is often prohibitively expensive. We tackle this problem by evaluating not only the standard quality metrics on downstream tasks but also the memory footprint and inference time. We present MOROCCO, a framework to compare language models compatible with \texttt{jiant} environment which supports over 50 NLU tasks, including SuperGLUE benchmark and multiple probing suites. We demonstrate its applicability for two GLUE-like suites in different languages.

==> old_text.tex <==
% \begin{itemize}
% \item SentEval\footnote{\url{https://github.com/facebookresearch/SentEval}} \cite{conneau2018senteval}
% \item GLUE\footnote{\url{https://gluebenchmark.com}} \cite{wang2018glue}
% \item SuperGLUE\footnote{\url{https://super.gluebenchmark.com}} \cite{wang2019superglue}
% \item decaNLP\footnote{\url{http://decanlp.com}} \cite{McCann2018decaNLP}
% \item LINSPECTOR \footnote{\url{https://linspector.ukp.informatik.tu-darmstadt.de}} \cite{eichler-etal-2019-linspector,DBLP:journals/corr/abs-1903-09442}
% % \item oLMpics CITE
% \end{itemize}


% The choice of the downstream tasks is straightforward and is limited to various sentiment classification, natural language inference, paraphrase detection and image captioning tasks. The downstream tasks are constructed from well-knows datasets. The probing tasks are meant to analyse morphological, syntactical and semantic information encoded in sentence embeddings.  From a technical perspective, SentEval is a python command line tool.  


% Secondly, the tasks exploited by the mentioned benchmarks are more of academic nature. The text sources can be thought of as being ``clean'' in that sense that they are free from grammatical errors and/or typos. For example, Microsoft Research Paraphrase Corpus, used in several benchmarks, has been complied from news headlines and thus has been spellchecked multiple times. In real life setup user-generated texts contain a lot of slang, code switching, emoticons and other informal language phenomena.

% We propose to make a competition for text embedding systems and include user-generated texts. The key idea here is to have some model which takes some text as input (the text is represented as character sequence) and outputs a dense vector representation of this text.%The robustness property which we are aiming to achieve for participating systems is described below.

Several benchmarks have been developed to evaluate and analyze word and sentence embeddings over the past few years. 
{\bf SentEval} \cite{conneau2018senteval} is one of the first frameworks intended to evaluate the quality of sentence embeddings. A twofold set of transfer tasks is used to assess the generalization power of sentence embedding models. The transfer tasks comprise downstream tasks, in which the sentence embedding is used as a feature vector, and probing tasks, which are aimed to evaluate the capability of sentence embeddings to encode linguistic properties. 


The {\bf General Language Understanding Evaluation (GLUE)} benchmark is a collection of tools for evaluating the performance of language models across a diverse set of existing natural language understanding tasks, adopted from different sources. These tasks are divided into two parts: single sentence classification tasks and sentence pair classifications tasks subdivided further into similarity and inference tasks. GLUE also includes a hand-crafted diagnostic test, which probes for complex linguistic phenomena, such as the ability of the model to express lexical semantics and predicate-argument structure, to poses logical apparatus and knowledge representation. GLUE benchmark is combined from a python tool and a publicly available leader board. GLUE provides with the train test splits for each task, so that a custom model can be learned on the train set and the predictions on the test set can be submitted to the leader board.  GLUE  is recognized as a de-facto standard benchmark to evaluate transformer-derived language models. The library called transformers \cite{Wolf2019HuggingFacesTS}, which provides the python interface to the state-of-the general-purpose language models, supports GLUE evaluation in a few lines of code. Last but not least, GLUE informs on human baselines for the tasks, so that the submitted models are compared not only to the baseline, but also to the human performance. The SuperGLUE \cite{wang2019superglue} follows GLUE paradigm for language model evaluation, providing with more complex tasks, of which some require reasoning capabilities and some are aimed at detecting ethical biases. 

{\bf decaNLP} \cite{McCann2018decaNLP} widens the scope for language model evaluation by introducing ten disparate natural language tasks. These tasks comprise text classification problems as well as sequence tagging and sequence transformation problems. The latter include machine translation and text summarization, while the former include semantic parsing and semantic role labelling. 

% Although decaNLP along with the associated research direction focuses on multi-task learning as a form of question answering, it supports zero-shot evaluation. Similarly to GLUE and SuperGLUE benchmarks, decaNLP exists in form of a python tool and a publicly available leader board.

It should be noted, that although covering a variety of NLP tasks, all of the aforementioned benchmarks focus on the English language. To the best of our knowledge, {\bf LINSPECTOR} is a first multi-lingual benchmark for evaluating the performance of language models. LINSPECTOR offers 22 probing tasks to analyse for a single linguistic feature such as case marking, gender, person, or tense for 52 languages. A part of these 22 probing tasks are static, i.e. are aimed at evaluation of word embeddings, and the rest are contextual and should be used to evaluate language models. In contrast to GLUE, SuperGLUE and decaNLP benchmarks, there is no leader board. Recent cross-lingual benchmarks, {\bf XTREME} and {\bf xGLUE} ...


% еще можно написать про DialoGLUE


\subsection{Novelty}

% \begin{table*}[]
% \centering
% \begin{tabular}{| p{2.8cm} | p{2.5cm} | p{1.5cm} | p{3.3cm} |} \hline
%           & tasks                        & leader board & what is scored    \\ \hline
% SentEval   & probing, downstream tasks  & no           & vector representations                    \\ \hline
% GLUE       & downstream tasks           & yes          & a file of predictions \\ \hline
% SuperGLUE  & downstream tasks           & yes          & a file of predictions \\ \hline
% decaNLP    & downstream tasks           & yes           & no                    \\ \hline
% LINSPECTOR & probing                    & no           & a model \\  \hline           
% \end{tabular}
% \caption{Characteristics of NLP benchmarks}
% \label{tab:comparison}
% \end{table*}

Table \ref{tab:comparison} presents with a technical comparison of the discussed benchmarks. Two significant drawbacks are common to them. First, unlike computer vision benchmarks \cite{gauen2017low} none of these benchmarks account for computational efficiency. 
